On the Capacity of Zero-Drift First Arrival Position Channels in Diffusive Molecular Communication

Recent advancements in understanding the impulse response of the first arrival position (FAP) channel in molecular communication (MC) have illuminated its Shannon capacity. While Lee et al. shed light on FAP channel capacities with vertical drifts, the zero-drift scenario remains a conundrum, primarily due to the challenges associated with the heavy-tailed Cauchy distributions whose first and second moments do not exist, rendering traditional mutual information constraints ineffective. This paper unveils a novel characterization of the zero drift FAP channel capacity for both 2D and 3D. Interestingly, our results reveal a 3D FAP channel capacity that is double its 2D counterpart, hinting at a capacity increase with spatial dimension growth. Furthermore, our approach, which incorporates a modified logarithmic constraint and an output signal constraint, offers a simplified and more intuitive formula (similar to the well-known Gaussian case) for estimating FAP channel capacity.

==> tempWords.tex <==
Certainly. Here's the revised paragraph with the new sentence integrated for clarity and coherence:

In the realm of FAP channels spanning \(n\)-dimensional spaces, the one-shot channel model is aptly portrayed using an additive vector form, as detailed in \cite{lee2022arrival}:
$
    \mathbf{x}_{\text{out}} = \mathbf{x}_{\text{in}} + \mathbf{x}_{\text{n}},
$
with \(\mathbf{x}_{\text{in}}\) symbolizing the releasing position, \(\mathbf{x}_{\text{out}}\) indicating the arriving position, and \(\mathbf{x}_{\text{n}}\) capturing the random position deviation resulting from propagation mechanisms. It's pivotal to understand that vectors \(\mathbf{x}_{\text{in}}\), \(\mathbf{x}_{\text{out}}\), and \(\mathbf{x}_{\text{n}}\) are members of the Euclidean vector space \(\mathbb{R}^{n-1}\); this is because one dimension is allocated for traversal, rendering it void of information-carrying capacity in that specific dimension. Previous studies have provided the probability density function of \(\mathbf{x}_{\text{n}}\) \cite{lee2016distribution,pandey2018molecular,lee2022arrival}, yet fully grasping the channel capacity for this unique position channel is an ongoing exploration. A seminal work by Lee et al. \cite{lee2023char} shed light on the FAP channel capacity in contexts with a positive vertical drift. Nonetheless, in zero-drift contexts, the conundrum of channel capacity remains. This paper ambitiously aims to fill this scholarly void by introducing robust formulas for the zero-drift FAP channel capacity across 2D and 3D spaces, incorporating an innovative logarithmic constraint, as elucidated in Sections~III and IV.

%%---------
Here's the revised version of the final paragraph of the Introduction:

The ensuing sections of this paper are organized in the following manner: Section~\ref{pre-A} provides a succinct review of mutual information and the Shannon channel capacity framework. Section~\ref{sec:CM} outlines the channel model under scrutiny and introduces the \(\alpha\)-power constraint. Our principal findings are delineated in Section~\ref{sec:MR}. The paper culminates with conclusions presented in Section~\ref{sec:conclude}.
%%-----------
Certainly. Here's an alternative:

The subsequent sections of this paper are organized as follows: Section~\ref{pre-A} offers a concise review of mutual information and the Shannon channel capacity framework. In Section~\ref{sec:CM}, we outline the channel model in focus and introduce the \(\alpha\)-power constraint. Our core findings are presented in Section~\ref{sec:MR}. We draw our conclusions in Section~\ref{sec:conclude}.


%%----
Here's the revised Conclusion section:

In this research, we dissect the capacity challenge posed by the zero-drift first arrival position (FAP) communication channel within diffusive molecular communication (MC) frameworks. Our investigation uncovers that as the drift velocity nears zero, both 2D and 3D FAP channels naturally simplify to their univariate and bivariate Cauchy distribution counterparts.

While recent studies such as \cite{lee2023char} have delved into the FAP channel capacity under conditions of positive \emph{vertical drift}, comprehending the Shannon capacity of FAP channels with \emph{zero drift}—or, in essence, multidimensional Cauchy channels—stands as an unresolved query at this juncture. This complex arena owes its intricacies to the Cauchy distribution's heavy-tailed attribute, positioning it within the expansive $\alpha$-stable distribution family, notable for their frequent absence of a second moment. Consequently, conventional constraints, such as the variance of random variables, falter when trying to articulate the signal space.

Navigating this complexity, we weave the concept of $\alpha$-power, a nuanced relative power measure, into molecular communication discussions. By outlining the signal space indispensable for understanding the no-drift FAP channel capacity, we extract the Shannon capacity for the FAP channel across both 2D and 3D domains in a definitive closed-form structure, underpinning it with a fresh logarithmic constraint. The capacity formulations articulated in Theorem~\ref{thm:T1} and Theorem~\ref{thm:T2} underscore an intriguing phenomenon: the 3D FAP channel's capacity eclipses its 2D counterpart by a factor of two when benchmarked against the identical dispersion parameter \(A\). This revelation amplifies the perspective that as spatial dimension \(n\) expands, FAP channels inherently harness greater informational bandwidth.
